A Brooks' Theorem for Triangle-Free Graphs

Let G be a triangle-free graph with maximum degree \delta(G). We show that the chromatic number \c{hi}(G) is less than 67(1 + o(1))\delta/ log \delta.

==> commands.tex <==
\usepackage{amsmath,amsfonts}
\newcommand{\KL}{\textup{KL}}
\newtheorem{observation}{Observation}
\newtheorem{Thm}{Theorem}
%\newtheorem{theorem}{Theorem}
%\newtheorem{lemma}[Thm]{Lemma}
\newtheorem{Cor}[Thm]{Corollary}
\newtheorem{Obs}[Thm]{Observation}
\newtheorem{Claim}[Thm]{Claim}
%\newtheorem{claim}{Claim}
%\newtheorem{lemma}{Lemma}
%\newtheorem{Observation}{Observation}
%\newtheorem{theorem}{Theorem}
%\newenvironment{proof}{\noindent {\sc Proof:}}{$\Box$ \smallskip}

\newtheorem{Ex}{Exercise}
\newtheorem{Exa}{Example}
\newtheorem{Rem}{Remark}

\newtheorem{Def}{Definition}
%\newtheorem{problem}{Problem}

\def\mindist{\Delta}
\def\mindistbar{\bar{\Delta}}
\def\sk{\smallskip}
\newcommand{\dist}[2]{{d_{#2}(#1)}}
\newcommand{\set}[1]{\{#1\}}
\newcommand{\zug}[2]{\langle #1,#2 \rangle}

\newcommand{\bone}{{\bf{1}}}

\newcommand{\He}{{\bf{He}}}
\newcommand{\JS}{{\bf{JS}}}
\newcommand{\calW}{{\mathcal{W}}}
\newcommand{\calS}{{\mathcal{S}}}
\newcommand{\calC}{{\mathcal{C}}}
\newcommand{\calD}{{\mathcal{D}}}
\newcommand{\calK}{{\mathcal{K}}}
\newcommand{\calF}{{\mathcal{F}}}
\newcommand{\calG}{{\mathcal{G}}}
\newcommand{\calH}{{\mathcal{H}}}
\newcommand{\calN}{{\mathcal{N}}}
\newcommand{\bbF}{{\bf{F}}}
\newcommand{\bbE}{{\bf{E}}}
\newcommand{\bbP}{{\bf{P}}}
\newcommand{\bbR}{{\bf{R}}}
\newcommand{\bbT}{{\bf{T}}}
\newcommand{\efdist}{{\bar{d}}}
\newcommand{\dt}{{\bf{dt}}}
\newcommand{\dx}{{\bf{dx}}}
\newcommand{\dr}{{\bf{dr}}}
\newcommand{\tx}{{\tilde{x}}}
\newcommand{\bbZ}{{\bf{Z}}}

\newcommand{\hvc}{{\sc{Correlation-Cluster}}}
\newcommand{\lvc}{{\sc{Low-Variance Cluster}}}
\newcommand{\lsc}{{\sc{Low-Separation Cluster}}}
\newcommand{\hvs}{{\sc{Correlation-Subspace}}}
\newcommand{\lvs}{{\sc{Low-Variance Subspace}}}
\newcommand{\tsvd}{{\sc{HT-SVD}}}
\newcommand{\tcor}{{\sc{HT-Correlations}}}
\newcommand{\tlsc}{{\sc{Low Separation Cluster}}}

\newcommand{\ccomp}{{\mathcal{C}_{\mathcal{F} \cup \mathcal{G}}}}
\newcommand{\nullsp}[1]{\bar{#1}}
\newcommand{\nccomp}{\bar{C}_{\calF \cup \calG}}
%\def\nullcenterf{\calN_\calF}
\def\nullcenterf{\bbP_\calF(\nullsp{\calC}_\calF)}

\def\nullcenterg{\bbP_\calG(\nullsp{\calC}_\calG)}

\def\ie{\textit{i.e.,}\ }
\newcommand{\cov}[2]{{\bf{Cov}}(#1,#2)}
\newcommand{\var}{{\bf{Var}}}
\newcommand{\Var}{{\bf{Var}}}
\newcommand{\Cov}{{\bf{Cov}}}
\newcommand{\Bin}{{\textbf{Bin}}}

\newcommand{\F}{\tilde{F}}
\newcommand{\G}{\tilde{G}}

%\newcommand{\pf}[1]{p_{#1}^{(f)}}
%\newcommand{\qf}[1]{q_{#1}^{(f)}}

\newcommand{\diff}{{\bf{diff}}}

\newcommand{\kcnote}[1]{{\sf{\textbf{$\clubsuit$ #1 $\clubsuit$}}}}

\newcommand{\Fs}{\bar{F}}
\newcommand{\Gs}{\bar{G}}
\newcommand{\EM}{\bar{M}}

% begin comment.sty ?
\makeatletter
\begingroup \catcode `|=0 \catcode `[= 1
\catcode`]=2 \catcode `\{=12 \catcode `\}=12
\catcode`\\=12 |gdef|@xcomment#1\end{comment}[|end[comment]]
|endgroup
\def\@comment{\let\do\@makeother \dospecials\catcode`\^^M=10\def\par{}}
\def\begincomment{\@comment\@xcomment}
\makeatother
\newenvironment{comment}{\begincomment}{}


\newcommand{\Repartition}{\textbf {Repartition}}
\newcommand{\score}{\textbf {Score}}

\newcommand{\kl}{{\bf{KL}}}
\newcommand{\tD}{{\tilde{D}}}


